Consensus-Based Set-Theoretic Control in Power Systems

Set-theoretic control is a useful technique for dealing with the uncertainty introduced into power systems by renewable energy resources. Although set operations are computationally expensive in large systems, distributed approaches serve as a remedy. In this paper, we propose a novel consensus-based approach for set-theoretic frequency control in power systems. A robust controlled-invariant set (RCI) for the system is generated by composing RCIs for each bus in the network. The process of generating these sets uses a consensus-based approach in order to facilitate discovery of mutually compatible subsystem RCIs. Each bus seeks to maximize the size of its own RCI while treating the effects of coupling as an unknown-but-bounded disturbance. The consensus routine, which demonstrates linear convergence, is embedded into a backwards reachability analysis of initial safe sets. Results for a 9-bus test case show that simple model predictive controllers associated with the resulting RCIs maintain safe operation when the system is subjected to worst case (adversarial) fluctuations in net demand, where conventional controllers are shown to fail.

==> scratch.tex <==
% Abstract: 

Set-theoretic control techniques are an active area of research in power systems due to their ability to guarantee safe operation in the face of significant uncertainty from renewable energy resources. However, the complexity of set computations in higher-dimensional spaces remains a barrier to widespread implementation. Distributed techniques improve scalability but at the cost of increased conservatism. In this paper, we carefully consider the




This is due to the variability in renewable energy supply, combined with the fact that renewables do not contribute to the system's mechanical inertia.   Distributed set-based control techniques improve scalability but at the cost of increased conservatism. In this paper, we propose a distributed set-based controller that reduces conservatism by accounting for several properties specific to the structure of power systems.

% Prelim: 

Consider two systems described by discrete dynamics \begin{align}
    x^+ &= f(x(t)) \label{eqn:nov4_1} \\
    x^+ &= f(x(t),u(t),d(t)) \label{eqn:nov4_2}
\end{align} where $x(t)$ is the state of the system at time $t$, $x^+$ is the state at time $t+1$, $u$ is a control input chosen from some set $\U \subseteq \R^m$, and $d$ is an exogenous disturbance chosen from a set $\D \in \R^p$. 

% Model:

Numerical results from a 9-bus test case show that the entries of $B_2$ are on the same order of magnitude as the entries of $B_1,$ meaning that the effects of coupled inputs represented by $B_2u$ are not negligible. Therefore, in a small power system, a real power injection at the terminals of generator $i$ has a non-negligible effect on the rotational frequency of all generators neighboring $i$.

The standard Kron reduction cannot be used since the algebraic buses have time-varying inputs and disturbances. 

The disturbances can be located anywhere in the system.

\begin{gather}
    \dot{x} = \underbrace{A_1x + B_1u}_\text{local dynamics} + \underbrace{A_2x + B_2u + Ed}_\text{non-local effects}
\end{gather}
where $A_1$ and $B_1$ are block-diagonal, $A_2 = \tilde{A}-A_1,$ and $B_2 = B - B_1.$

$A_{1i}$ and $B_{1i}$ are the block diagonal elements of $A_1$ and $B_1$, and $A_{2i},B_{2i},$ and $E_i$ are matrices formed from the $i$th block-row and the $j$th block-columns of $A_2, B_2,$ and $E$ for all $j \in \N_i$.

The system is decomposed into $N_G$ subsystems described by 

the system equations \begin{align}
    x_i^+ =& (I+hA_{1i})x_i(t) +hB_{1i}u_i(t) \nonumber \\
    &+ (I+hA_{2i})x(t) + hB_{2i}u_{\N_i}(t) + hEd(t) \\.
\end{align}

This model refers disturbances and inputs to the synchronous generator rotors assuming a DC power flow model and swing equation dynamics, with the DC power flow assumption modified such 

We assume all sets are 0-symmetric C-sets (meaning that they are convex, compact, contain the origin as an interior point, and that if $x \in \X,$ then $-x \in \X$).

After decomposition into subsystems, it is tempting to treat the disturbance $d \in \R^{N_L}$ at each bus as acting independently. However, since each bus sees the same $d$, this is an overly conservative approximation. To rectify this, we redefine dynamics with respect to a slack bus. A new coordinate system is defined as \begin{subequations}\label{eqn:nov5_3}
    \begin{align}
    z_1 &= x_1\\
    z_i &= x_i - x_1 , i = 2,...,N_G
    \end{align}
\end{subequations} This invertible coordinate transformation, denoted by the linear operator $Q$, gives rise to system matrices $\bar{A}_1 = QA_1Q^{-1}, \bar{B}_1 =  QB_1,$ and the others defined similarly. Indeed, it can be observed in a 9-bus test case that the elements of $\bar{E}$ are smaller than those of $E$, reflecting the fact that disturbances $d$ have a smaller impact on the relative states $z$ than on the absolute states $x$.


% Algorithm:

When the system dynamics are linear and the sets $\X,\U,$ and $\D$ are polytopes, all operations in Algorithm \ref{alg:backprop} generate polytopes, and computations are tractable if the dimension is not too high.

The goal is to design a feedback controller that guarantees safe operation under any sequence of disturbances. Further, we seek to maximize robustness to initial conditions.

Due to the choice of discretization, $\S$ is an inner approximation of the continuous-time maximal RCI \cite{Blanchini2015}.

beginning with the safe set $\X$ and iteratively constructing 1-step admissible sets to generate $k$-steps admissible sets denoted $\X^{(k)}$.  When $k = \infty$, we obtain the largest RCI contained in $\X$.

One problem with computing the RCI in this way is that subsystems will ``compete'' for leeway. Each subsystem seeks to maximize the size of its own RCI, but in doing so, subjects its neighbors to the possibility of larger coupling disturbances. Larger coupling disturbances force each RCI to shrink. We propose a fixed-point iteration which resembles a consensus subroutine in order to find, for each iteration in Algorithm \ref{alg:alg1}, a set of $k+1$-steps admissible sets for each subsystem
% Need to explain this better
    % Reduces conservatism perspective
    % Competitive perspective
    % Necessary extension of algorithm 1 perspective (need to know what the coupling disturbances are)
, starting from the set of $k$-steps admissible sets $\{Z_i^{(k)}\}_{i=1}^{N_G}$, if the sets $\Y_i^{(k)}$ are nonempty for all $i$, then the sets $\Y_i^{(k,l)} \rightarrow \Y_i^{(k)}, l = 1,2,...$ converge 

First, the target set is narrowed in order to account for unknown-but-bounded disturbances. Then, the set of states that can be driven to the target set in one time step is computed.

% Control design:
Each controller is of the form $u_i = u_i(x_i), i = 1,...,N_G$, meaning that each controller can only measure local states $x_i$ and take actions using the locally available power injection $u_i.$

